Modelling thermochemical processes in protoplanetary disks I: numerical methods

The dispersal phase of planet-forming disks via winds driven by irradiation from the central star and/or magnetic fields in the disk itself is likely to play an important role in the formation and evolution of planetary systems. Current theoretical models lack predictive power to adequately constrain observations. We present PRIZMO, a code for evolving thermochemistry in protoplanetary disks capable of being coupled with hydrodynamical and multi-frequency radiative transfer codes. We describe the main features of the code, including gas and surface chemistry, photochemistry, microphysics, and the main cooling and heating processes. The results of a suite of benchmarks, which include photon-dominated regions, slabs illuminated by radiation spectra that include X-ray, and well-established cooling functions evaluated at different temperatures show good agreement both in terms of chemical and thermal structures. The development of this code is an important step to perform quantitative spectroscopy of disk winds, and ultimately the calculation of line profiles, which is urgently needed to shed light on the nature of observed disk winds.

==> general.tex <==



